MPE inference using an Incremental Build-Infer-Approximate Paradigm

Exact inference of the most probable explanation (MPE) in Bayesian networks is known to be NP-complete. In this paper, we propose an algorithm for approximate MPE inference that is based on the incremental build-infer-approximate (IBIA) framework. We use this framework to obtain an ordered set of partitions of the Bayesian network and the corresponding max-calibrated clique trees. We show that the maximum belief in the last partition gives an estimate of the probability of the MPE assignment. We propose an iterative algorithm for decoding, in which the subset of variables for which an assignment is obtained is guaranteed to increase in every iteration. There are no issues of convergence, and we do not perform a search for solutions. Even though it is a single shot algorithm, we obtain valid assignments in 100 out of the 117 benchmarks used for testing. The accuracy of our solution is comparable to a branch and bound search in majority of the benchmarks, with competitive run times.

==> old.tex <==
\step{\it Local max-marginalization:~ (lines 11-34 of Algorithm \ref{alg:ApproximateCTF})}\label{sec:trimLargeCliques}
The goal of this step is to bring down sizes of these cliques to $mcs_{im}$, \textcolor{blue}{while preserving the joint distribution of the interface variables as much as possible. The idea is to remove non-interface variables that are least correlated with the interface variables} from a minimal set of cliques in $CTF_a$, with the following constraints.
\begin{enumerate}
\item [(a)] Resulting $CTF_a$ remains valid.
\item [(b)] Each connected  CT $\in CTF_a$  remains connected. %This is essential for computation of the partition function and posterior beliefs.
\end{enumerate}
\textcolor{red}{Modify.}
{\color{blue}
To do this, we define a metric based on pairwise mutual information ($MI$) between variables in a clique. Let $IV_C$ and $NIV_C$ denote the set of interface and non-interface variables in a clique $C$. For all variables in the clique, we define the \textit{Maximum Local Mutual Information, $MLMI$} as follows
\begin{equation}
   MLMI_{n,C} =
  \begin{cases}
    \max\limits_{\forall x\in {IV_C}} MI(n;x) &  n\in NIV_C \\
   %  \max\limits_{\forall x\in {IV_C} \setminus n} MI(n;x) &  n\in IV_C\\
     \max\limits_{\forall x\in {C \setminus n}} MI(n;x) &  n\in IV_C
    \end{cases}
\end{equation}
where
\begin{align*}
          MI(x;y) &= \sum\limits_{s \in D_x, w \in D_y} p(s,w) \log \frac{p(s,w)}{p(s)p(w)}
\end{align*}
\begin{align*}
\color{red}
          M(x;y)&= \sum\limits_{s \in D_x, w \in D_y} p(s,w) \log \frac{p(s,w)}{max(p(s),p(w))}
\end{align*}
For a non-interface variables, $MLMI$ of a net is the maximum $MI$ between the net and  interface variables in the clique. $MLMI$ for an interface variables is defined as the  maximum $MI$ between the net and  all the other variables in the clique.

The \textit{Maximum Mutual Information, $maxMI$} for both types of variables is defined as the maximum $MLMI$ over all cliques, given as
	\begin{align}
	maxMI_n=\max_{\forall C\in CTF ~s.t. ~n\in C} MLMI_{n,C}
	\end{align}
}
\textcolor{red}{Remove all MI, MLMI, maxMI logic and say we prefer to remove nets present in fewer cliques, branch selection - branch with largest number of containing cliques??}

$CTF_a$ is first simplified by \textit{locally max-marginalizing} out non-interface variables from individual large cliques while retaining them in as many smaller sized cliques consistent with RIP. By local max-marginalization, we mean the following. Assume that a node $n$ is present in two adjacent cliques $C_i$ and $C_j$, and in the corresponding sepset $S_{i,j}$. Local marginalization results in two approximate cliques $C_i' = C_i\setminus n$ and $C_j'=C_j\setminus n$ with sepset $S_{i,j}' = S_{i,j}\setminus n$. The corresponding beliefs are
        \begin{align*}
          \beta(C_i') &= \max\limits_{n.states}\beta(C_i), \\ \beta(C_j')  &= \max\limits_{n.states}\beta(C_j), \\ \mu(S_{i,j}') &=  \max\limits_{n.states}\mu(S_{i,j})
        \end{align*}
The nets chosen for local max-marginalization are ones with the least $maxMI$, since these nets have the lowest $MI$ with the interface variables.

The steps involved in performing local marginalization are as follows. The line numbers in the following description correspond to those in Algorithm ~\ref{alg:ApproximateCTF}. 
We first identify the set of large cliques with size $>mcs_{im}$  and store them in a list $L_c$ (line xx).  The metrics $maxMI,~MLMI$ are computed for all variables in $L_c$ (line xx). Then, we find the set of non-interface variables present in these cliques and add them to a list $N$ (line xx). We start with the node $n$ that has the least $maxMI$. %In case of a tie, we prefer the node present in fewer cliques. 
In order to retain $n$ in as many cliques as possible, we find the list of cliques containing $n$ with size $\leq mcs_{im}$  and store them in a list $L_s$ (lines xx). 
Next, we identify the subgraph of $CTF_a$ corresponding to cliques in $L_s$ and divide it into a set of disjoint subtrees, $L_{st}$ (line xx).    
Net $n$ is retained in the subtree that contains the clique with largest $MLMI$, denoted as $L_r$ (line xx). In case of a tie, we choose the subtree with the largest number of cliques.
Net $n$ is locally marginalized out from all other containing cliques and sepsets, while ensuring each connected CT remains connected (lines xx). 
Any resultant non-maximal clique is removed, and its neighbors are connected to the containing clique.

Figure \ref{fig:approxStep3} shows an example of this step. The non-interface net $n_2$ is locally marginalized out from three of the cliques, while it is retained in the other two cliques.

Once this is done, if there are cliques with size $> mcs_{im}$, they will contain only interface variables and non-interface variables that cannot be removed without breaking a connected CT.
The interface variables are added to the list $N$ (line xx) and following the same procedure as for NIVs, the interface variable is retained in the subtree that contains the clique with largest $MLMI$.

However, there is one difference (lines xx).  
An interface variable must be contained in at least one clique in $CTF_a$. If there are no cliques with size $\leq mcs_{im}$ containing a particular interface variable, the algorithm proceeds to the next variable without doing anything. 
This is because we require a connected CT to remain connected.

==> tables/old/bkp.tex <==
% 75-25-5 &458 &2 &6 &-20.84/-20.84 &-20.84/-18.25 &N/-19.99 &N/-19.73 \\
% & & & &(3) &(520) &(327) &(235) \\
% 75-26-5 &462 &2 &6 &-21.89/-21.89 &-21.89/-18.51 &N/-20.43 &-23.06/-21.38 \\
% & & & &(4) &(3600) &(417) &(270) \\
% 90-20-5 &232 &2 &2 &-5.70/-5.70 &-5.70/-4.67 &N/-5.45 &-6.62/-5.63 \\
% & & & &(1) &(0) &(186) &(122) \\
% 90-30-5 &282 &2 &5 &-13.12/-13.12 &-13.12/-10.20 &N/-11.88 &N/-11.95 \\
% & & & &(4) &(1428) &(456) &(378) \\
% 90-34-5 &377 &2 &3 &-13.29/-13.29 &-13.29/-10.92 &N/-12.88 &N/-12.63 \\
% & & & &(4) &(898) &(645) &(489) \\
% 90-38-5 &642 &2 &11 &-19.87/-19.87 &N/-14.72 &N/-18.24 &N/-17.13 \\
% & & & &(13) &(3600) &(906) &(581) \\
% 90-42-5 &365 &2 &9 &-20.94/-20.94 &N/-15.81 &N/-19.32 &N/-19.14 \\
% & & & &(16) &(3600) &(1101) &(751) \\
% 90-46-5 &1215 &2 &10 &-28.32/-28.31 &0.00/-19.93 &N/-23.62 &N/-24.82 \\
% & & & &(13) &(3600) &(1324) &(923) \\

% &BN\_76 &24 &N/-186.59 &-209.14$^{1}$/-171.99 &N/-173.03 &N/-174.54 &3600 &2311 &1256 & 176 \\
% &BN\_75 &27 &N/-135.94 &N/-125.20 &N/-126.91 &N/-125.66 &3600 &3600 &2206 & 135\\
%&BN\_72 &22 &-193.89* &N &N &N  &3600 &3600 &2570 &141\\
% &BN\_71 &23 &-157.85/-155.59 &N/-132.79 &N/-138.53 &N/-136.44 & 3600 &1785 &471 & 129 \\
% &BN\_73 &21 &-171.80/-167.44 &-180.98/-158.92 &N/-160.27 &N/-160.44 &3600 &3600 &2079 &140 \\
% &BN\_72 &22 &-193.89*/-196.35 &N/-175.31 &N/-178.05 &N/-180.30  &3600 &3600 &2570 &141\\

%&BN\_70 &21 &-126.62*/-127.57 &-136.58**/-105.06 &N/-97.56 &N/-105.27 &138 &3600 &2606 & 1306 \\

==> tables/old/delta.map.tex <==
\begin{table*}[!htp]\centering
\caption{Comparison of error in max-marginal over non-evidence variables and probability of MAP assignment ($X^*$) obtained using IBIA with $mcs_p=20$ and WMB with $ibound=20,10$. Entries are marked with `-' if the probability obtained is 0 and with `err' if inference fails. \textcolor{blue}{Metric for choice of variables to be trimmed $\rightarrow$Ascending order of number of cliques}}
\scriptsize
\begin{tabular}{|c|c|ccc|ccc|c|}\toprule
\multirow{2}{*}{\textbf{CKT}} &\multirow{2}{*}{$\mathbf{MaxMarg_{Exact}}$} &\multicolumn{3}{c|}{$\mathbf{MaxMarg_{Alg}-MaxMarg_{Exact}}$} &\multicolumn{3}{c|}{$\mathbf{P(X_{Alg}^*)-P(X_{Exact}^*)}$} &\textbf{\#Partitions} \\\cmidrule{3-9}
& &\textbf{WMB20 (UB)} &\textbf{WMB10 (UB)} &\textbf{IBIA} &\textbf{WMB20} &\textbf{WMB10} &\textbf{IBIA} &\textbf{IBIA} \\\midrule
BN\_1 &-17.74 &2.46 &2.78 &0 &0 &-5.94 &0 &3 \\
BN\_101 &-23.18 &0 &0.55 &0.07 &0 &-2.88 &-0.01 &3 \\
BN\_103 &-36.54 &1.71 &2.13 &0 &0 &-2.31 &0 &2 \\
BN\_11 &-25.41 &6.8 &6.99 &0 &0 &-1.30 &0 &2 \\
BN\_115 &-7.94 &0.63 &3.06 &0.04 &0 &-5.93 &-1.51 &4 \\
BN\_12 &-15.12 &0.51 &0.93 &0.05 &-0.09 &-3.02 &-1.08 &4 \\
BN\_126 &-56.01 &0 &0.86 &0 &-28.40 &-46.25 &0 &19 \\
BN\_127 &-58.30 &3.83 &1.29 &0 &-53.65 &-2.84 &0 &19 \\
BN\_128 &-47.42 &0 &0 &0 &0 &-12.60 &0 &18 \\
BN\_129 &-62.16 &4.43 &4.05 &-0.18 &-39.66 &-71.64 &-4.05 &15 \\
BN\_13 &-19.71 &0.34 &1.07 &0 &-0.71 &-4.07 &0 &6 \\
BN\_130 &-58.26 &1.56 &0.03 &0 &-61.82 &-44.47 &0 &18 \\
BN\_131 &-54.64 &0.13 &2.36 &0.24 &-41.02 &-43.92 &0 &17 \\
BN\_132 &-65.70 &8.46 &8.39 &0.56 &-39.37 &-38.76 &-6.92 &13 \\
BN\_133 &-54.34 &2.61 &3.48 &0.8 &-40.02 &-21.36 &-1.54 &17 \\
BN\_134 &-56.95 &0.81 &1.94 &-0.17 &-26.17 &-58.29 &0 &15 \\
BN\_14 &-20.91 &2.18 &2.18 &0.01 &0 &0 &0 &3 \\
BN\_15 &-20.33 &0.93 &1.33 &0.2 &-2.87 &-1.85 &-1.11 &6 \\
BN\_16 &-0.85 &0.01 &0.01 &0 &0 &0 &0 &12 \\
BN\_17 &-0.85 &0.01 &0.01 &0 &0 &0 &0 &10 \\
BN\_18 &-0.85 &0.01 &0.01 &0 &0 &0 &0 &10 \\
BN\_19 &-0.85 &0.01 &0.01 &0 &0 &0 &0 &11 \\
BN\_2 &-18.73 &1.69 &2.47 &0 &0 &-2.67 &0 &2 \\
BN\_42 &-18.06 &0.3 &0.3 &0 &0 &- &- &3 \\
BN\_43 &-18.06 &0 &0 &0 &0 &- &- &2 \\
BN\_45 &-18.06 &0 &0 &0 &0 &- &- &3 \\
BN\_47 &-4.21 &0 &0 &0 &- &- &0 &3 \\
BN\_48 &-4.21 &0 &0 &0 &- &- &0 &3 \\
BN\_55 &-9.63 &0 &0 &0 &- &- &0 &3 \\
BN\_57 &-9.63 &0.3 &0.3 &0 &- &- &0 &2 \\
BN\_58 &-9.63 &0.3 &0.3 &0 &- &- &0 &2 \\
BN\_7 &-15.79 &1.07 &1.13 &0 &0 &-1.73 &0 &2 \\
BN\_8 &-16.15 &0.06 &0.37 &0 &-1.24 &-2.40 &0 &3 \\
BN\_86 &-1.48 &0.35 &0.35 &0 &0 &0 &0 &2 \\
BN\_87 &-1.48 &0.35 &0.35 &0 &0 &0 &0 &2 \\
BN\_9 &-16.87 &0.43 &0.59 &-0.02 &0 &-0.35 &-0.02 &4 \\
BN\_90 &-1.48 &0.01 &0.01 &0 &0 &0 &0 &3 \\
BN\_91 &-1.48 &0.01 &0.01 &0 &0 &0 &0 &2 \\
BN\_92 &-1.48 &0.05 &0.05 &0 &0 &0 &0 &2 \\
BN\_93 &-1.48 &0.05 &0.05 &0 &0 &0 &0 &2 \\
BN\_95 &-19.48 &0 &0.45 &0 &0 &-2.49 &0 &2 \\
BN\_97 &-18.23 &0 &1.07 &0 &0 &-2.46 &0 &3 \\
BN\_99 &-20.45 &2.41 &3.29 &0 &0 &-3.00 &0 &3 \\
pedigree1 &-45.58 &0 &0.07 &0 &0 &-0.45 &0 &2 \\
pedigree13 &-73.37 &2.22 &3.36 &1.23 &-11.09 &- &- &11 \\
pedigree18 &-125.25 &0 &2.31 &0 &0.00 &- &-1.32 &6 \\
pedigree20 &-53.79 &err &0.75 &0 &err &- &-3.65 &4 \\
pedigree23 &-62.39 &err &0.63 &0 &err &- &0 &3 \\
pedigree25 &-160.84 &1.91 &2.39 &-0 &-3.82 &- &-2.86 &5 \\
pedigree30 &-136.95 &0.12 &3.71 &0 &-2.71 &- &-1.32 &6 \\
pedigree33 &-74.95 &4.38 &8.33 &-0 &- &- &-1.91 &3 \\
pedigree39 &-155.61 &1.45 &3.6 &-0.15 &0 &- &- &5 \\
pedigree44 &-96.97 &2.95 &4.46 &0.93 &-7.63 &- &-0.59 &8 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/old/exact.bkp.tex <==
\begin{table}[tb]\centering
\caption{Comparison of errors in log probabilities of MPE assignments ($\Delta_{MAP}$) obtained using different methods.  $p$ denotes the number of partitions obtained with IBIA. Entries are marked as `N' if either no solution is obtained in 1hr or the probability of the solution obtained is zero.}\label{tab:deltaMap.exact}
\scriptsize
\setlength\tabcolsep{2pt}
\begin{tabular}{lrrrrrrrrrr}\toprule
\multirow{2}{*}{} &\multirow{2}{*}{\bf Network} &\multirow{2}{*}{\bf p} &\multicolumn{4}{c}{$\mathbf{\Delta_{MAP}}$} &\multicolumn{4}{c}{\textbf{Runtime}} \\\cmidrule{4-11}
& & &IBIA &AOBB &WMB &JGLP &AOBB &WMB &JGLP &IBIA \\\midrule
% \multirow{4}{*}{\bf \rom{1}} &BN\_19 &16 &0 &0 &0 &0 &1 &433 &329 &32 \\
% &BN\_17 &12 &0 &0 &0 &0 &0 &404 &315 &31 \\
% &BN\_12 &4 &-0.38 &0 &-0.09 &-0.28 &0 &74 &66 &1 \\
% &pedigree39 &5 &0 &0 &0 &0 &16 &770 &633 &6 \\ \midrule
\multirow{12}{*}{\bf \rom{1}} &BN\_127 &19 &0 &0 &-53.65 &0 &0 &242 &216 &13 \\
&BN\_133 &17 &0 &0 &-40.02 &0 &0 &247 &231 &14 \\
&BN\_131 &17 &0 &0 &-41.02 &0 &0 &220 &205 &13 \\
&BN\_134 &15 &0 &0 &-26.17 &0 &0 &245 &232 &12 \\
&BN\_130 &18 &0 &0 &-61.82 &-0.17 &1 &239 &243 &10 \\
&BN\_126 &19 &0 &0 &-28.40 &-19.48 &1 &208 &193 &13 \\
&BN\_129 &15 &0 &0 &-39.66 &-6.40 &0 &196 &216 &10 \\
&BN\_132 &13 &-0.31 &0 &-39.37 &-4.65 &37 &237 &228 &9 \\
&BN\_15 &6 &-0.09 &0 &-2.87 &-0.66 &0 &106 &72 &1 \\
&pedigree30 &6 &0 &0 &-2.71 &0 &7 &260 &423 &14 \\
&pedigree44 &8 &0 &0 &-7.63 &-0.97 &492 &816 &1318 &6 \\
&pedigree13 &11 &-1.27 &0 &-11.09 &-1.68 &3600 &1215 &571 &10 \\
\midrule
\multirow{10}{*}{\bf \rom{2}} &BN\_60 &6 &0 &0 &N&N&41 &391 &271 &3 \\
&BN\_74 &10 &0 &0 &N&N&798 &50 &270 &9 \\
&pedigree23 &3 &0 &0 &N&N&0 &25 &3600 &1 \\
&pedigree42 &7 &-0.09 &0 &N&N&273 &63 &731 &3 \\
&pedigree7 &10 &-0.37 &0 &N&-2.68 &3600 &3600 &2467 &10 \\
&pedigree9 &9 &-0.95 &0 &N&-1.03 &379 &808 &513 &10 \\
&pedigree34 &10 &-1.18 &0 &N&N&3600 &1505 &3601 &8 \\
&pedigree41 &9 &-1.06 &0 &N&N&3600 &47 &3601 &8 \\
&pedigree33 &3 &-1.91 &0 &N&-0.80 &6 &2276 &460 &3 \\
&pedigree31 &13 &-2.25 &-0.45 &N&-3.34 &3600 &3601 &1743 &12 \\
% \rowcolor{gray!20}&75-26-5 &6 &-21.89 &-21.89 &N&-23.06& 3600 &417 &270 & 4 \\
% \rowcolor{gray!20}&90-20-5 &2 &-5.70 &-5.70 &N &-6.62 &0 &186 &122 &1  \\
% \rowcolor{gray!20}&75-25-5 &6 &-20.84 &-20.84 &N &N & 520 &327 &235 & 3 \\
% \rowcolor{gray!20}&90-30-5 &5 &-13.12 &-13.12 &N &N &1428 &456 &378 &4  \\
% \rowcolor{gray!20}&90-34-5 &3 &-13.29 &-13.29 &N &N &898 &645 &489 &4 \\
\midrule


% \rowcolor{gray!20}&90-38-5 &11 &-19.87 &N &N &N &3600 &906 &581  &13\\
% \rowcolor{gray!20}&90-42-5 &9 &-20.94 &N &N &N &3600 &1101 &751 &16 \\
% \rowcolor{gray!20}&90-46-5  &10 &-28.32 &N &N &N &3600 &1324 &923 &13  \\
% \rowcolor{gray!20}&90-50-5 &13 &-29.16 &N &N &N  &3600 &1547 &1055 &24 \\
&pedigree40 &11 &-1.88 &-7.89 &N&N&3600 &90 &196 &12 \\
\multirow{-2}{*}{\bf \rom{3}}&pedigree51 &10 &0 &-4.68 &N&-2.30 &3600 &1866 &750 &11 \\
% \midrule
% \multirow{5}{*}{\bf \rom{4}} &BN\_42 &3 &N&0 &0 &0 &0 &57 &36 &1 \\
% &BN\_43 &2 &N&0 &0 &0 &0 &104 &49 &1 \\
% &BN\_54 &6 &N&0 &N&0 &0 &308 &192 &2 \\
% %&BN\_69 &11 &N&0 &N&N&1815 &130 &484 &? \\
% &BN\_64 &7 &N&0 &N&N&1 &417 &228 &? \\
% &BN\_77 &7 &N&0 &N&N&586 &14 &176 &13 \\
% %&pedigree19 &11 &N&-3.49 &N&N&3600 &18 &627 &? \\
% \midrule
% \rowcolor{gray!20}&BN\_76 &24 &N &N &N &N &3600 &2311 &1256 & 176 \\
% \rowcolor{gray!20}&BN\_75 &27 &N &N &N &N &3600 &3600 &2206 & 135\\
% \multirow{-3}{*}{\bf \rom{5}} &&&&&&&&\\
\bottomrule
\end{tabular}
\end{table}



==> tables/old/mapCmp.noexact.tex <==
\begin{table}[!htp]\centering
\caption{Comparison of maximum probability assignment and overall max-marginal estimate obtained using different methods. For methods MBE-MM, WMB and JGLP, the upper bound is used as an estimate for max-marginal. $v$ is the number of non-evidence variables, $k$ is the maximum domain size and $p$ is the number of partitions obtained with IBIA. 
%Parameters used: IBIA, $mcs_p=20$, AOBB:$ibnd=10$, WMB and JGLP: $ibnd=10$ for BN\_UAI and $ibnd=20$ for grid-BN.
}\label{tab: }
\scriptsize
\setlength\tabcolsep{1.5pt}
\begin{tabular}{lcccrrrrr}\toprule
\multirow{2}{*}{\textbf{Network}} &\multirow{2}{*}{\textbf{v}} &\multirow{2}{*}{\textbf{k}} &\multirow{2}{*}{\textbf{p}} &\multicolumn{4}{c}{\textbf{$\mathbf{P(X^{*}_{Alg})~/ ~MaxMarg_{Alg}}$  (Runtime)}} \\\cmidrule{5-8}
& & & &\textbf{IBIA} &\textbf{AOBB+MBE-MM} &\textbf{WMB} &\textbf{JGLP} \\\midrule

75-25-5 &458 &2 &6 &-20.84/-20.84 &-20.84/-18.25 &N/-19.99 &N/-19.73 \\
& & & &(3) &(520) &(327) &(235) \\
75-26-5 &462 &2 &6 &-21.89/-21.89 &-21.89/-18.51 &N/-20.43 &-23.06/-21.38 \\
& & & &(4) &(3600) &(417) &(270) \\
90-20-5 &232 &2 &2 &-5.70/-5.70 &-5.70/-4.67 &N/-5.45 &-6.62/-5.63 \\
& & & &(1) &(0) &(186) &(122) \\
90-30-5 &282 &2 &5 &-13.12/-13.12 &-13.12/-10.20 &N/-11.88 &N/-11.95 \\
& & & &(4) &(1428) &(456) &(378) \\
90-34-5 &377 &2 &3 &-13.29/-13.29 &-13.29/-10.92 &N/-12.88 &N/-12.63 \\
& & & &(4) &(898) &(645) &(489) \\
90-38-5 &642 &2 &11 &-19.87/-19.87 &N/-14.72 &N/-18.24 &N/-17.13 \\
& & & &(13) &(3600) &(906) &(581) \\
90-42-5 &365 &2 &9 &-20.94/-20.94 &N/-15.81 &N/-19.32 &N/-19.14 \\
& & & &(16) &(3600) &(1101) &(751) \\
90-46-5 &1215 &2 &10 &-28.32/-28.31 &0.00/-19.93 &N/-23.62 &N/-24.82 \\
& & & &(13) &(3600) &(1324) &(923) \\
90-50-5 &1152 &2 &13 &-29.16/-29.16 &N/-21.47 &N/-27.11 &N/-25.69 \\
& & & &(24) &(3600) &(1547) &(1055) \\
\bottomrule
\end{tabular}
\end{table}

==> tables/old/metricCmp.tex <==
\begin{table*}[!htp]\centering
\caption{Comparison of metrics for choice of variables to be trimmed.\\ M1=Ascending order of number of cliques\\
M2=$M(X;Y)= \sum\limits_{s \in D_X, w \in D_Y} p(s,w) \log \frac{p(s,w)}{max(p(s),p(w))}$ \\where,~ $p(s)=max_Y P(X=s, Y),~p(w)=max_X P(X, Y=w)$}\label{tab:metricCmp}
\scriptsize
\begin{tabular}{lrrrrrrr}\toprule
\multirow{2}{*}{} &\multicolumn{2}{c}{$\mathbf{MaxMarg_{ibia} - MaxMarg_{exact}}$} &\multicolumn{2}{c}{$\mathbf{P(X^{*}_{ibia})-P(X^{*}_{exact})}$} &\multicolumn{2}{c}{\textbf{\#Partitions}} \\\cmidrule{2-7}
&\textbf{M1} &\textbf{M2; tiebreak=M1} &\textbf{M1} &\textbf{M2; tiebreak=M1} &\textbf{M1} &\textbf{M2; tiebreak=M1} \\\midrule
pedigree1 &0 &0 &0 &0 &2 &2 \\
pedigree13 &1.23 &0.91 & & &11 &14 \\
pedigree18 &0 &0 &-1.32 &-2.27 &6 &7 \\
pedigree19 &2.13 &1.55 & & &11 &12 \\
pedigree20 &0 &0 &-3.65 &-5.22 &4 &4 \\
pedigree23 &0 &0 &0 &0 &3 &4 \\
pedigree25 &0 &-0 &-2.86 &-3.82 &5 &5 \\
pedigree30 &0 &0 &-1.32 &-1.32 &6 &7 \\
pedigree31 &0.58 &0.38 & & &13 &14 \\
pedigree33 &0 &-0 &-1.91 &-0.95 &3 &4 \\
pedigree34 &0.34 &0.45 & & &10 &10 \\
pedigree37 &1.26 &0.95 & &-0.70 &5 &5 \\
pedigree38 &0.15 &0.15 & &-5.57 &4 &6 \\
pedigree39 &-0.15* &-0 & & &5 &7 \\
pedigree40 &\bf 3.1* &\bf -1.84 & & &7 &12 \\
pedigree41 &0.92 &1.56 & & &9 &9 \\
pedigree42 &0.06 &0.03 & & &7 &6 \\
pedigree44 &0.93 &-0.17 &-0.59 & &8 &9 \\
pedigree50 &0 &-0 & & &6 &8 \\
pedigree51 &-0.2 &-0 & & &10 &10 \\
pedigree7 &\bf 1.54 &\bf 2.33 & & &10 &12 \\
pedigree9 &1.32 &0.95 & & &9 &11 \\
BN\_126 &0 &-0 &0 &0 &19 &19 \\
BN\_127 &0 &0 &0 &0 &19 &18 \\
BN\_128 &0 &0 &0 &0 &18 &19 \\
BN\_130 &0 &0 &0 &0 &18 &15 \\
BN\_131 &0.24 &0 &0 &0 &17 &15 \\
BN\_133 &0.80 &-0.03 &-1.54 &0 &17 &19 \\
BN\_129 &-0.18 &-0.18 &-4.05 &-8.08 &15 &16 \\
BN\_134 &-0.17 &0 &0 &0 &15 &16 \\
BN\_132 &0.56 &0.88 &-6.92 &-2.36 &13 &18 \\
BN\_16 &0 &-0 &0 &0 &12 &10 \\
BN\_19 &0 &-0 &0 &0 &11 &16 \\
BN\_69 &0.80 &1.03 &- &- &11 &16 \\
BN\_17 &0 &-0 &0 &0 &10 &12 \\
BN\_18 &0 &-0 &0 &0 &10 &10 \\
BN\_71 &Err:exactNotKnown* &Err:exactNotKnown &- &- &9 &24 \\
BN\_63 &0 &0 &- &- &7 &7 \\
BN\_64 &0 &0 &- &- &7 &7 \\
BN\_13 &0 &-0 &0 &0 &6 &7 \\
BN\_15 &0.20 &0.16 &-1.11 &-1.40 &6 &6 \\
BN\_53 &0 &0 &- &- &6 &6 \\
BN\_54 &0 &0 &- &- &6 &6 \\
BN\_60 &0 &0 &- &- &6 &6 \\
BN\_66 &0 &0 &- &- &6 &6 \\
BN\_67 &0 &0 &- &- &6 &6 \\
BN\_68 &0 &0 &- &- &6 &6 \\
BN\_77 &\bf 7.36* &\bf 3.50* &- &- &6 &12 \\
BN\_59 &0 &0 &- &- &5 &5 \\
BN\_65 &0 &0 &- &- &5 &5 \\
BN\_74 &0.46* &0.51 &- &- &5 &5 \\
BN\_115 &0.04 &0 &-1.51 &0 &4 &4 \\
BN\_12 &0.05 &0.17 &-1.08 &-1.09 &4 &3 \\
BN\_9 &-0.02 &-0.02 &-0.02 &-0.47 &4 &4 \\
BN\_1 &0 &0 &0 &0 &3 &3 \\
BN\_101 &0.07 &-0 &-0.01 &0 &3 &2 \\
BN\_14 &0.01 &0.01 &0 &0 &3 &3 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/old/noExact.bkp.tex <==
\begin{table}[!htbp]\centering
\caption{Comparison of the logarithm of MPE assignment probabilities obtained with different methods. $p$ denotes the number of partitions obtained with IBIA. Entries are marked as `N' if either no solution is obtained in 1hr or the probability of the solution obtained is zero.\textcolor{red}{Fix runtimes. Add number of iterations. Count number of testcases in each category.}}\label{tab:map.noexact}
\scriptsize
\setlength\tabcolsep{2pt}
\begin{tabular}{lrrrrrrrrrr}\toprule
\multirow{2}{*}{} &\multirow{2}{*}{\bf Network} &\multirow{2}{*}{\bf p} &\multicolumn{4}{c}{$\log P(X^{*}_{Alg})$} &\multicolumn{4}{c}{\textbf{Runtime}} \\\cmidrule{4-11}
& & &IBIA &AOBB &WMB &JGLP &AOBB &WMB &JGLP &IBIA \\\midrule
\multirow{9}{*}{\bf \rom{1}}&75-21-5 &3 &-13.28 &-13.28 &N &-13.37 &21 &229 &140 &2 \\
&90-20-5 &2 &-5.70 &-5.70 &N &-6.62 &0 &186 &122 &1  \\
&75-22-5 &5 &-15.61 &-15.61 &N &-16.46 &6 &227 &168 &1 \\
&75-23-5 &6 &-15.43 &-15.43 &N &-16.40 &82 &299 &188 &2 \\
&75-24-5 &5 &-16.08 &-16.08 &N &-16.87 &37 &331 &211 &2 \\
&75-26-5 &6 &-21.89 &-21.89 &N&-23.06& 3600 &417 &270 & 4 \\
&75-25-5 &6 &-20.84 &-20.84 &N &N & 520 &327 &235 & 3 \\
&90-30-5 &5 &-13.12 &-13.12 &N &N &1428 &456 &378 &4  \\
&90-34-5 &3 &-13.29 &-13.29 &N &N &898 &645 &489 &4 \\
\midrule
\multirow{8}{*}{\bf \rom{2}}&BN\_72 &22 &-193.89 &N &N &N  &3600 &3600 &2570 &141\\
&BN\_70 &21 &-126.62 &-136.58 &N &N  &3600 &2606 & 1306 &138 \\
&BN\_71 &23 &-157.85 &N &N &N & 3600 &1785 &471 & 129 \\
&BN\_73 &21 &-169.45 &-180.98 &N &N &3600 &3600 &2079 &140 \\
&90-38-5 &11 &-19.87 &N &N &N &3600 &906 &581  &13\\
&90-42-5 &9 &-20.94 &N &N &N &3600 &1101 &751 &16 \\
&90-46-5  &10 &-28.32 &N &N &N &3600 &1324 &923 &13  \\
&90-50-5 &13 &-29.16 &N &N &N  &3600 &1547 &1055 &24 \\
% &pedigree40 &11 &-1.88 &-7.89 &N&N&3600 &90 &196 &12 \\
% \rowcolor{gray!20}
%  &BN\_71 &23 &-157.85 &N &N &N & 3600 &1785 &471 & 129 \\
% \rowcolor{gray!20}&BN\_73 &21 &-171.80 &-180.98 &N &N &3600 &3600 &2079 &140 \\
% \midrule
% \multirow{5}{*}{\bf \rom{4}} &BN\_42 &3 &N&0 &0 &0 &0 &57 &36 &1 \\
% &BN\_43 &2 &N&0 &0 &0 &0 &104 &49 &1 \\
% &BN\_54 &6 &N&0 &N&0 &0 &308 &192 &2 \\
% %&BN\_69 &11 &N&0 &N&N&1815 &130 &484 &? \\
% &BN\_64 &7 &N&0 &N&N&1 &417 &228 &? \\
% &BN\_77 &7 &N&0 &N&N&586 &14 &176 &13 \\
% %&pedigree19 &11 &N&-3.49 &N&N&3600 &18 &627 &? \\
% \midrule
% \rowcolor{gray!20}&BN\_76 &24 &N &N &N &N &3600 &2311 &1256 & 176 \\
% \rowcolor{gray!20}&BN\_75 &27 &N &N &N &N &3600 &3600 &2206 & 135\\
% \multirow{-3}{*}{\bf \rom{5}} &&&&&&&&\\
\bottomrule
\end{tabular}
\end{table}

==> tables/old/table.allCategories.tex <==
\begin{table*}[!htp]\centering
\caption{Comparison of errors in log probabilities of MAP assignments obtained using different methods. $p$ denotes the number of partitions obtained with IBIA. Entries are marked as `N' if either no solution is obtained in 1hr or the probability of the solution obtained is zero.}\label{tab:deltaMap}
\scriptsize
\setlength\tabcolsep{2pt}
\begin{tabular}{lrrrrrrrrrr}\toprule
\multirow{2}{*}{} &\multirow{2}{*}{\bf Network} &\multirow{2}{*}{\bf p} &\multicolumn{4}{c}{$\mathbf{\Delta_{MAP}/PX^{*}}$} &\multicolumn{4}{c}{\textbf{Runtime}} \\\cmidrule{4-11}
& & &IBIA &AOBB &WMB &JGLP &AOBB &WMB &JGLP &IBIA \\\midrule
\multirow{4}{*}{\bf \rom{1}} &BN\_19 &16 &0 &0 &0 &0 &1 &433 &329 &32 \\
&BN\_17 &12 &0 &0 &0 &0 &0 &404 &315 &31 \\
&BN\_12 &4 &-0.38 &0 &-0.09 &-0.28 &0 &74 &66 &1 \\
&pedigree39 &5 &0 &0 &0 &0 &16 &770 &633 &6 \\ \midrule
\multirow{5}{*}{\bf \rom{2}} &BN\_127 &19 &0 &0 &-53.65 &0 &0 &242 &216 &13 \\
&BN\_133 &17 &0 &0 &-40.02 &0 &0 &247 &231 &14 \\
&BN\_131 &17 &0 &0 &-41.02 &0 &0 &220 &205 &13 \\
&BN\_134 &15 &0 &0 &-26.17 &0 &0 &245 &232 &12 \\
&pedigree30 &6 &0 &0 &-2.71 &0 &7 &260 &423 &14 \\ \midrule
\multirow{20}{*}{\bf \rom{3}} &BN\_130 &18 &0 &0 &-61.82 &-0.17 &1 &239 &243 &10 \\
&BN\_126 &19 &0 &0 &-28.40 &-19.48 &1 &208 &193 &13 \\
&BN\_129 &15 &0 &0 &-39.66 &-6.40 &0 &196 &216 &10 \\
&BN\_132 &13 &-0.31 &0 &-39.37 &-4.65 &37 &237 &228 &9 \\
&BN\_15 &6 &-0.09 &0 &-2.87 &-0.66 &0 &106 &72 &1 \\
&BN\_60 &6 &0 &0 &N&N&41 &391 &271 &3 \\
&BN\_74 &10 &0 &0 &N&N&798 &50 &270 &9 \\
&pedigree44 &8 &0 &0 &-7.63 &-0.97 &492 &816 &1318 &6 \\
&pedigree13 &11 &-1.27 &0 &-11.09 &-1.68 &3600 &1215 &571 &10 \\
&pedigree7 &10 &-0.37 &0 &N&-2.68 &3600 &3600 &2467 &10 \\
&pedigree9 &9 &-0.95 &0 &N&-1.03 &379 &808 &513 &10 \\
&pedigree33 &3 &-1.91 &0 &N&-0.80 &6 &2276 &460 &3 \\
&pedigree31 &13 &-2.25 &-0.45 &N&-3.34 &3600 &3601 &1743 &12 \\
&pedigree23 &3 &0 &0 &N&N&0 &25 &3600 &1 \\
&pedigree42 &7 &-0.09 &0 &N&N&273 &63 &731 &3 \\
&pedigree41 &9 &-1.06 &0 &N&N&3600 &47 &3601 &8 \\
&pedigree34 &10 &-1.18 &0 &N&N&3600 &1505 &3601 &8 \\
\rowcolor{gray!20}&75-26-5 &6 &-21.89 &-21.89 &N&-23.06& 3600 &417 &270 & 4 \\
\rowcolor{gray!20}&90-20-5 &2 &-5.70 &-5.70 &N &-6.62 &0 &186 &122 &1  \\
\rowcolor{gray!20}&75-25-5 &6 &-20.84 &-20.84 &N &N & 520 &327 &235 & 3 \\
\rowcolor{gray!20}&90-30-5 &5 &-13.12 &-13.12 &N &N &1428 &456 &378 &4  \\
\rowcolor{gray!20}&90-34-5 &3 &-13.29 &-13.29 &N &N &898 &645 &489 &4 \\
\midrule
\rowcolor{gray!20}
 &BN\_71 &23 &-157.85 &N &N &N & 3600 &1785 &471 & 129 \\
\rowcolor{gray!20}&BN\_73 &21 &-171.80 &-180.98 &N &N &3600 &3600 &2079 &140 \\
\rowcolor{gray!20}&90-38-5 &11 &-19.87 &N &N &N &3600 &906 &581  &13\\
\rowcolor{gray!20}&90-42-5 &9 &-20.94 &N &N &N &3600 &1101 &751 &16 \\
\rowcolor{gray!20}&90-46-5  &10 &-28.32 &N &N &N &3600 &1324 &923 &13  \\
\rowcolor{gray!20}&90-50-5 &13 &-29.16 &N &N &N  &3600 &1547 &1055 &24 \\
&pedigree40 &11 &-1.88 &-7.89 &N&N&3600 &90 &196 &12 \\
\multirow{-8}{*}{\bf \rom{4}}&pedigree51 &10 &0 &-4.68 &N&-2.30 &3600 &1866 &750 &11 \\
\midrule
\multirow{5}{*}{\bf \rom{5}} &BN\_42 &3 &N&0 &0 &0 &0 &57 &36 &1 \\
&BN\_43 &2 &N&0 &0 &0 &0 &104 &49 &1 \\
&BN\_54 &6 &N&0 &N&0 &0 &308 &192 &2 \\
%&BN\_69 &11 &N&0 &N&N&1815 &130 &484 &? \\
&BN\_64 &7 &N&0 &N&N&1 &417 &228 &? \\
&BN\_77 &7 &N&0 &N&N&586 &14 &176 &13 \\
%&pedigree19 &11 &N&-3.49 &N&N&3600 &18 &627 &? \\
\midrule
\multirow{2}{*}{\bf \rom{6}}&BN\_76 &24 &N &N &N &N &3600 &2311 &1256 & 176 \\
&BN\_75 &27 &N &N &N &N &3600 &3600 &2206 & 135\\
\bottomrule
\end{tabular}
\end{table*}



==> tikz/approximateCTF.tex <==
\tikzstyle{circ}=[
circle,
minimum size=0.75cm,
draw=black,
inner sep=1pt,
%thick,
]
\begin{figure*}[!htb]
	\centering
%	\captionsetup[subfigure]{position=b}
	\begin{subfigure}[t]{0.5\textwidth}
			\centering
	\begin{tikzpicture}[scale=0.8, every node/.style={scale=0.8},highlightfill/.style={fill,rounded corners=1em, line width=1.5em,opacity=0.1,cap=round},]
	\node[circ] (c2) at (0,0){\color{gray}$\mathbf{n_1}$};
	\node (d2) at (0,0.7){\color{gray}$C_2$};
	\node[circ] (c1) at (-1.5,0){\color{blue}$\mathbf{i_1i_2}$};
	\node (d1) at (-1.5,0.7){\color{gray}$C_1$};
	\node[circ] (c3) at (1.5,-1.5){\color{gray}$\mathbf{n_1}$};
	\node (d3) at (1.8,-0.8){\color{gray}$C_3$};
	\node[circ] (c4) at (0,-3){\color{gray}$\mathbf{n_1}$};
	\node (d4) at (0,-3.7){\color{gray}$C_4$};
	\node[circ] (c5) at (-1.5,-3){\color{blue}$\mathbf{i_3}$};
	\node (d5) at (-1.5,-3.7){\color{gray}$C_5$};
%	\node[circ, fill=orange!20] (c6) at (3,-1.5){\color{gray}$\mathbf{n_1}$};
	\node[circ] (c7) at (4.5,-1.5){};
	\node (d6) at (4.5,-0.8){\color{gray}$C_6$};
	\node[circ] (c8) at (6,-1.5){};
	\node (d6) at (6.5,-0.8){\color{gray}$C_7$};
	\node[circ] (c9) at (6,-3){\color{blue}$\mathbf{i_6}$};
	\node (d6) at (6,-3.7){\color{gray}$C_8$};
	\node[circ] (c10) at (6,0){};
	\node (d6) at (6,0.7){\color{gray}$C_9$};
	\node[circ] (c11) at (4.5,0){\color{blue}$\mathbf{i_4}$};
	\node (d6) at (4.5,0.7){\color{gray}$C_{10}$};
	\node[circ] (c12) at (3,0){\color{blue}$\mathbf{i_4i_5}$};
	\node (d6) at (3,0.7){\color{gray}$C_{11}$};
	\draw (c1)--(c2);
	\draw (c2)--(c3);
	\draw (c3)--(c4);
	\draw (c4)--(c5);
%	\draw (c3)--(c6);
%	\draw (c6)--(c7);
	\draw (c3)--(c7);
	\draw (c7)--(c8);
	\draw (c8)--(c9);
	\draw (c8)--(c10);
	\draw (c10)--(c11);
	\draw (c11)--(c12);
	\drawoutside[highlightfill, black]{(c2.north) -- (c3.east) -- (c4.south)  -- cycle}
	\end{tikzpicture}
	\caption{\small Minimal subgraph of $CTF_{in}$ connecting interface nodes (Step1). The interface variables present in each clique are highlighted in blue.}
	\label{fig:approxStep1}
	\end{subfigure}\hfill{}%
	\begin{subfigure}[t]{0.48\textwidth}
			\centering
	\begin{tikzpicture}[scale=0.8, every node/.style={scale=0.8}]
	\node[circ,draw=white] (c2) at (0,0){};
		\node (d) at (0,-0.8){\color{gray}${C_{2}}'$};
	\node[circ, fill=gray!30] (cn2) at (0,-1.5) {};
	\node (tn2) [align=center, below=0.1 of cn2, xshift=0.9cm] { \bf \color{blue} Marginalize  $\mathbf{n_1}$};
	\node[circ] (c1) at (-1.5,0){};
	\node[circ] (c5) at (-1.5,-3){};
	%\node[circ, fill=orange!20] (c6) at (2,-1.5){};
	%\node (t6) [align=center, below=0.1 of c6, xshift=0.1cm] {\scriptsize \bf \color{blue}Marg. $\mathbf{n_2}$};
	\node[circ] (c7) at (3.5,-1.5){\color{gray} $\mathbf{n_2}$};
	\node (t7) [align=center, above=0.05 of c7] { \small \color{black!80} $cs=10$};
	\node[circ] (c8) at (5,-1.5){\color{gray} $\mathbf{n_2}$};
	\node (t8) [align=center, above right=0.05 of c8] {\small \color{black!80} $cs=15$};
	\node[circ] (c9) at (5,-3){};
	\node (t9) [align=center, right=0.05 of c9] {};
	\node[circ] (c10) at (5,0){\color{gray} $\mathbf{n_2}$};
	\node (t10) [align=center, above=0.05 of c10, xshift=1cm] {\bf \small \color{red} $cs=16$};
	\node[circ] (c11) at (3.5,0){\color{gray} $\mathbf{n_2}$};
	\node (t11) [align=center, above=0.05 of c11] {\small  \color{black!80} $cs=10$};
	\node[circ] (c12) at (2,0){\color{gray} $\mathbf{n_2}$};
	\node (t12) [align=center, above=0.05 of c12, xshift=-1cm] { \small \color{black!80} $cs=10$};
	\draw (c1)--(cn2);
	\draw (cn2)--(c5);
%	\draw (cn2)--(c6);
%	\draw (c6)--(c7);
	\draw (cn2)--(c7);
	\draw (c7)--(c8);
	\draw (c8)--(c9);
	\draw (c8)--(c10);
	\draw (c10)--(c11);
	\draw (c11)--(c12);
	\end{tikzpicture}
	\caption{\small $CTF_a$ obtained after exact marginalization of non-interface variables (Step2). All cliques containing $n_1$ are collapsed before marginalization.}
	\label{fig:approxStep2}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{0.48\textwidth}
			\centering
	\begin{tikzpicture}[scale=0.8, every node/.style={scale=0.8}]
	\node[circ,draw=white] (c2) at (0,0){};
	\node[circ] (cn2) at (0,-1.5) {};
	\node (d) at (0,-0.8){\color{gray}${C_{2}}'$};
	\node[circ] (c1) at (-1.5,0.25){};
	\node (d) at (-1,0.95){\color{gray}${C_{1}}'$};
	\node[circ] (c5) at (-1.5,-3){};
	\node (d) at (-0.8,-3){\color{gray}${C_{5}}'$};
%	\node[circ] (c6) at (2,-1.5){};
%	\node (d) at (2,-0.8){\color{gray}${C_{4}}'$};
	\node[circ] (c7) at (3.5,-1.5){\color{gray} $\mathbf{n_2}$};
	\node (d) at (3.5,-0.8){\color{gray}${C_{6}}'$};
	\node (t7) [align=center, below=0.01 of c7] {\small \color{black!80} $cs=10$};
	\node[circ] (c8) at (5,-1.5){\color{gray} $\mathbf{n_2}$};
	\node (d) at (5.5,-0.8){\color{gray}${C_{7}}'$};
	\node (t8) [align=center, below right=0.01 of c8] {\small \color{black!80} $cs=15$};
	\node[circ] (c9) at (5,-3){};
	\node (d) at (5.5,-2.5){\color{gray}${C_{8}}'$};
	\node[circ, draw=blue] (c12) at (2,0.25){};
	\node (d) at (1.7,0.95){\color{gray}${C_{11}}'$};
	\node[circ, draw=blue] (c10) at (5,0.25){};
	\node (t10) [align=center, below right=0.02 of c10] {\small \color{blue}  $cs=15$ };
	\node (d) at (5.5,0.95){\color{gray}${C_{9}}'$};
	\node[circ, draw=blue] (c11) at (3.5,0.25){};	
	\node (d) at (3.9,0.95){\color{gray}${C_{10}}'$};
	\node (t12) [align=center, below=0 of c11] {\small \color{blue}  $cs=9$ };
	\node (t12) [align=center, below=0 of c12] {\small \color{blue} $cs=9$ };
	\draw (c1)--(cn2);
	\draw (cn2)--(c5);
%	\draw (cn2)--(c6);
%	\draw (c6)--(c7);
	\draw (cn2)--(c7);
	\draw (c7)--(c8);
	\draw (c8)--(c9);
	\draw (c8)--(c10);
	\draw (c10)--(c11);
	\draw (c11)--(c12);
	\node (tm) [align=center,above=0.5 of c11] {\color{blue} \bf Marginalize $\mathbf{n_2}$};
	\draw [->, dotted, blue, thick](tm)--(c10.north);
	\draw [->, dotted, blue, thick](tm)--(c11.north);
	\draw [->, dotted, blue, thick](tm)--(c12.north);
	\end{tikzpicture}
	\caption{\small After local marginalization of variables from large cliques (Step3). Non-interface variable $n_2$ is locally marginalized from a subset of containing cliques to meet clique size constraint.}
	\label{fig:approxStep3}
	\end{subfigure}\hfill
% \begin{subfigure}[t]{0.48\textwidth}
% \centering
% \begin{tikzpicture}[scale=0.8, every node/.style={scale=0.8},highlightfill1/.style={fill, rounded corners=1em, line width=1em,cap=round,},]
% \node (c1) [align=center]{$C_1$};
% \node (c2) [align=center, right=0.1 of c1]{$C_2$};
% \node (c3) [align=center, right=0.1 of c2]{$C_3$};
% \node (c4) [align=center, right=0.1 of c3]{$C_4$};
% \node (c5) [align=center, right=0.1 of c4]{$C_5$};
% \node (c6) [align=center, right=0.1 of c5]{$C_6$};
% \node (c7) [align=center, right=0.1 of c6]{$C_7$};
% \node (c8) [align=center, right=0.1 of c7]{$C_8$};
% \node (c9) [align=center, right=0.1 of c8]{$C_9$};
% \node (c10) [align=center, right=0.1 of c9]{$C_{10}$};
% \node (c11) [align=center, right=0.1 of c10]{$C_{11}$};
% \node (cp1) [align=center, below=1 of c1]{${C_1}'$};
% \node (cp2) [align=center, below=1 of c3]{${C_2}'$};
% \node (cp5) [align=center, below=1 of c5]{${C_5}'$};
% \node (cp6) [align=center, below=1 of c6]{${C_6}'$};
% \node (cp7) [align=center, below=1 of c7]{${C_7}'$};
% \node (cp8) [align=center, below=1 of c8]{${C_8}'$};
% \node (cp9) [align=center, below=1 of c9]{${C_9}'$};
% \node (cp10) [align=center, below=1 of c10]{${C_{10}}'$};
% \node (cp11) [align=center, below=1 of c11]{${C_{11}}'$};
% \node (d) [align=center, below=1.5 of cp11] {};
% \draw [dashed,ultra thick, color=black] (c1)--(cp1);
% \draw [dashed,ultra thick, color=black] (c2)--(cp2);
% \draw [dashed,ultra thick, color=black] (c3)--(cp2);
% \draw [dashed,ultra thick, color=black] (c4)--(cp2);
% \draw [dashed,ultra thick, color=black] (c5)--(cp5);
% \draw [dashed,ultra thick, color=black] (c6)--(cp6);
% \draw [dashed,ultra thick, color=black] (c7)--(cp7);
% \draw [dashed,ultra thick, color=black] (c8)--(cp8);
% \draw [dashed,ultra thick, color=black] (c9)--(cp9);
% \draw [dashed,ultra thick, color=black] (c10)--(cp10);
% \draw [dashed,ultra thick, color=black] (c11)--(cp11);
% \drawoutside[highlightfill1, teal,opacity=0.2]{(c1.north west) -- (c11.north east) -- (c11.south east) -- (c1.south west) -- cycle};
% \drawoutside[highlightfill1, black,opacity=0.1]{(cp1.north west) -- (cp11.north east) -- (cp11.south east) -- (cp1.south west) -- cycle};
% \node (cin) [align=center, above=0.25 of c6] {$\mathbf{CTF_{in}}$};
% \node (a)[align=center, below=0.25 of cp6] {$\mathbf{CTF_{a}}$};
% \end{tikzpicture}
% \caption{Addition of links between cliques in $CTF_{in}$ and $CTF_a$ (Step4). }
% \label{fig:links1}
% \end{subfigure}
	\caption{Illustration of the proposed approach to approximate the partition CTF. Each circle represents a clique. A subset of clique scopes is indicated inside each clique. While $i_1,~i_2,~i_3,~i_4,~i_5$ are interface variables, $n_1,~n_2$ are non-interface variables. \textcolor{red}{Rescale/Discard?}}
\label{fig:approxCTF}
\end{figure*}


